Poor-Supervised Evaluation for SuperLLM via Mutual Consistency

The guidance from capability evaluations has greatly propelled the progress of both human society and Artificial Intelligence. However, as LLMs evolve, it becomes challenging to construct evaluation benchmarks for them with accurate labels on hard tasks that approach the boundaries of human capabilities. To credibly conduct evaluation without accurate labels (denoted as poor-supervised evaluation), we propose the PoEM framework. We first prove that the capability of a model can be equivalently assessed by the consistency between it and certain reference model, when their prediction distributions are independent and the sample size is infinite. To alleviate the insufficiencies of the conditions in reality, we further introduce an algorithm that treats humans (when available) and the models under evaluation as reference models, alternately conducting model weights calibration and filtering during E-step and M-step. Comprehensive experiments across 3 types of tasks with 16 mainstream LLMs have shown that PoEM under poor supervision can achieve an average of 0.98 Pearson correlation coefficient with supervised evaluation results, demonstrating good effectiveness, efficiency and generalizability. More generally, PoEM has advanced the evaluation paradigm evolution from human-centric to human&model-centric by treating both of them as reference models, mitigating the limitations of human evaluation in the era of LLMs.

==> discussion.tex <==
\section{Discussion}
\paragraph{Tasks With Open-ended Label Domain.} 
The experiments above have verified the effectiveness of $\mathcal{F}_{WEEM}$ in various tasks within closed label domain. Meanwhile, open-domain text generation is also an important aspect of LLM capability assessment. Unlike closed domain tasks holding a one-to-one relationship between input and output, open-domain tasks can have multiple appropriate answers for a given input. Therefore, evaluation based on consistency may not be suitable for open-domain evaluation and current mainstream methods depend on human-evaluator and LLM-evaluator \cite{geval}.
However, we still need a method to judge the capability of the LLM-evaluators when their capability surpass that of human-evaluator. The output of the LLM-evaluator is closed-domain, where we can use $\mathcal{F}_{EMEM}$ to carry out such evaluations, as demonstrated in \S\ref{exp2}. To summarize, $\mathcal{F}_{WEEM}$ can enhance the accuracy of model capability assessment in open-domain tasks by aiding in the selection of SuperEvaluators.

==> limitation.tex <==
\section*{Limitations}
\begin{enumerate}
\item We think there are 2 limitations of this paper:
The experiments above have verified the effectiveness of $\mathcal{F}_{PEEM}$ in various tasks within closed label domain. Meanwhile, open-domain text generation is also an important aspect of LLM capability assessment. Unlike closed domain tasks holding a one-to-one relationship between input and output, open-domain tasks can have multiple appropriate answers for a given input. Therefore, evaluation based on consistency may not be suitable for open-domain evaluation and current mainstream methods rely on human-evaluator and LLM-evaluator \citep{geval}.
However, we still need a method to choose the most capable evaluator. The output of certain evaluator is closed-domain, where we can use $\mathcal{F}_{PEEM}$ to carry out such evaluations, as demonstrated in \S\ref{exp2}. To summarize, $\mathcal{F}_{PEEM}$ can enhance the accuracy of model capability assessment in open-domain tasks by aiding in the selection of evaluators.
\item theory
\end{enumerate}



==> preliminary.tex <==
\section{Preliminary}
\subsection{Task Definition}
Given LLMs $\{\mathcal{M}^i\}^L_{i=1}$, datasets $\mathbb{D}: (X=\{x_i\}^N_{i=1},Y=\{y_i\}^N_{i=1})$ and predictions of $\mathcal{M}^i$ on $X$ as $\hat{Y}^i=\{\hat{y}^i_j\}^N_{j=1}$, the consistency between $\{\hat{Y}^i\}_{i=1}^L$ and true labels $Y$, denoted as $\{Cons(\hat{Y}^i,Y)\}^L_{i=1}$, shortened to $B \in \mathcal{R}^{L}$, is the accurate measurement of the capabilities of these LLMs. Our research aims to assess LLMs when $Y$ is unavailable. Therefore, we consider designing a mapping algorithm $\mathcal{F}$ that can map LLM predictions $\{\hat{Y}^i\}_{i=1}^L$ (with inaccurate human annotations if available) to capability vector $\hat{B}\in \mathcal{R}^{L}$
, where $\hat{B}_i$ can substitute for $B_i$ in evaluating the capabilities of model $\mathcal{M}^i$. We calculate the correlation coefficient between $\hat{B}$ and $B$ to validate the effectiveness of $\mathcal{F}$. It should be noted that the calculation method of $Cons(\cdot)$ depends on the label domain, which we will introduce in \S\ref{exp}.

\subsection{Intuition of Theorem~\ref{theorem1}}
We propose Theorem~\ref{theorem1} to credibly implement poor-supervised evaluation, which is grounded in an intuition that is straightforward to understand: For the samples where the reference model predicts correctly, strong model tends to have higher consistency with the reference model compared to weak model, $Cons(\mathcal{M}^{strong},\dot{\mathcal{M}})$$>Cons(\mathcal{M}^{weak},\dot{\mathcal{M}})$. While for the samples where the reference model predicts incorrectly, if the reference model does not tend to make the same predictions as either strong or weak models, the consistency of both strong and weak model with the reference model should be the same, $Cons(\mathcal{M}^{strong},\dot{\mathcal{M}})$$= Cons(\mathcal{M}^{weak},\dot{\mathcal{M}})$. Therefore, across all the samples, $Cons(\mathcal{M}^{strong},\dot{\mathcal{M}})$$>Cons(\mathcal{M}^{weak},\dot{\mathcal{M}})$. 

% The predictions of a model can be considered as the true labels with noise. At this point, the consistency between two models can also be seen as the consistency of one of the models with the noised true labels. Bared this in mind, we attempt to prove that under certain conditions, the noise can be ignored and the consistency among models is equivalent to the consistency between models and the true labels.

% % \begin{theorem}
% % \label{theorem1}
% % For given models $\mathcal{M}_1,\mathcal{M}_2,\mathcal{M}_3$ and their predictions on $\{x_i\}^N$, $Cons(\hat{Y}^1,Y) < Cons(\hat{Y}^2,Y) \Leftrightarrow Cons(\hat{Y}^1,\hat{Y}^3) < Cons(\hat{Y}^2,\hat{Y}^3)$ holds when:
% % \begin{itemize}[leftmargin=20pt]
% % \setlength{\itemsep}{0pt}
% % \setlength{\parsep}{0pt}
% % \setlength{\parskip}{0pt}
% % \item Condition 1: $N \to \infty$;
% % \item Condition 2: Both $(P(\hat{y}^1|x),P(\hat{y}^3|x))$ and $(P(\hat{y}^2|x),P(\hat{y}^3|x))$ are independently distributed;
% % \item Condition 3: $\mathcal{M}_3$ performs better than random predictor.
% % \end{itemize}
% % \end{theorem}
% We prove the theorem both in the continuous and discrete label domains in Appendix~\ref{theorem_proof}. The theorem proposed above supports our intuition that we can use the consistency between models to measure their capabilities under the above conditions.

% However, although $Condition\ 3$ can be assumed to be satisfied by default, $Condition\ 1$ and $2$ cannot be completely fulfilled in real scenarios. Some LLMs (such as Llama-series, as we will demonstrate later) may have a higher affinity, meaning they might be prone to make the same types of errors; thus, their predictions will be non-independently distributed to some extent. Moreover, constrained by sampling costs, $N$ must inevitably be finite. Therefore, conducting unsupervised evaluations under such circumstances can be very challenging.

\begin{figure*}[!htb]
    \centering
    \subfigure[Consistency Matrix]{\includegraphics[width=0.49\hsize, height=0.38\hsize]{img/Cons_Precalculus.pdf}\label{fig: sub_figure1}} 
    \subfigure[Affinity Matrix]{\includegraphics[width=0.49\hsize, height=0.38\hsize]{img/Bias_Precalculus.pdf} \label{fig: sub_figure2}}
    \setlength{\belowcaptionskip}{0pt}
    \caption{Inter-model consistency matrix and affinity matrix on MATH-Precalculus dataset among 16 LLMs.}
    \label{fig:explore}
\end{figure*}

\subsection{Visualization of Consistency and Affinity}
Although Condition 2 can be assumed to be satisfied naturally, Condition 1 and 3 cannot be completely fulfilled in real scenarios as discussed before.
To explore the impact of the insufficiency of Condition 1 and 3 in real scenarios, we visualize the consistency matrix $C$ and the affinity matrix $A$ of models to be evaluated.
$C_{i,j}$ $\in$ [0,1] denotes $Cons(\hat{Y}^i,\hat{Y}^j)$, the average consistency between the predictions of $\mathcal{M}^i$ and $\mathcal{M}^j$ on $X$. And $A_{i,j}$ $\in$ [-1,1] reflects the affinity of $\mathcal{M}^i$ to $\mathcal{M}^j$, which can be calculated as follows:
\begin{equation}
\label{eq:pre-1}
% \small
A_{i,j} = \frac{C_{i,j}}{Sum(C_{i})} - \frac{B_j}{Sum(B)}
\end{equation}
A positive $A_{i,j}$ implies using $\mathcal{M}^i$ as the reference model to estimate $\hat{B}_j$ will overestimate the performance of $\mathcal{M}^j$ and vice versa.

We conduct this preliminary experiment on subset Precalculus of MATH \cite{MATH} benchmark with 16 LLMs (See detailed setup in \S\ref{sec:exp1setup}). 
As shown in Figure~\ref{fig: sub_figure1}, the top 16 rows demonstrate  the $C$, the third-to-last row calculates $\{Avg(C_i)\}_{i=1}^L$, the penultimate row shows $B$, while the $i^{th}$ column of the last row represents the Pearson coefficient between $C_i$ and $B$ (the closer to 1, the stronger the linear correlation). 
% From Figure~\ref{fig: sub_figure1}, we note that due to the insufficient fulfillment of Condition 1 and 3, $C_i$ cannot fully replace $B$ especially for weaker $\mathcal{M}^i$.
From Figure~\ref{fig: sub_figure1}, we can observe the following tendencies and corresponding insights.
(1) The third-to-last and penultimate row show a positive correlation $\rightarrow$ \textit{\textbf{Insight 1}}: \textit{stronger models tend to have higher consistency with other models};
(2) The last and penultimate row also show a positive correlation $\rightarrow$ \textit{\textbf{Insight 2}}: \textit{stronger models' consistency with other models can better reflect the true performance of these models.}
Considering that model predictions tend to converge towards the true labels and predictions of stronger models are closer to the true labels, the above two insights are natural and reasonable.

From Figure~\ref{fig: sub_figure2}, we confirm that some LLMs belonging to the same series (Llama-2 series, MetaMath series) indeed exhibit mutual affinity, which makes their consistency biased to reflect their true performance. Furthermore, we observe \textit{\textbf{Insight 3}}: \textit{weaker models tend to exhibit higher affinity.} We attribute this to the consistency between weak models and strong models underestimating the performance of the strong models, indirectly leading to a higher affinity among weak models. More generally, the proportion of samples correctly predicted by a weak model is too low, using it as a reference model may not suffice to differentiate between strong and weak models.



